Beyond Sequence: Impact of Geometric Context for RNA Property Prediction

Accurate prediction of RNA properties, such as stability and interactions, is crucial for advancing our understanding of biological processes and developing RNA-based therapeutics. RNA structures can be represented as 1D sequences, 2D topological graphs, or 3D all-atom models, each offering different insights into its function. Existing works predominantly focus on 1D sequence-based models, which overlook the geometric context provided by 2D and 3D geometries. This study presents the first systematic evaluation of incorporating explicit 2D and 3D geometric information into RNA property prediction, considering not only performance but also real-world challenges such as limited data availability, partial labeling, sequencing noise, and computational efficiency. To this end, we introduce a newly curated set of RNA datasets with enhanced 2D and 3D structural annotations, providing a resource for model evaluation on RNA data. Our findings reveal that models with explicit geometry encoding generally outperform sequence-based models, with an average prediction RMSE reduction of around 12% across all various RNA tasks and excelling in low-data and partial labeling regimes, underscoring the value of explicitly incorporating geometric context. On the other hand, geometry-unaware sequence-based models are more robust under sequencing noise but often require around $2-5\times$ training data to match the performance of geometry-aware models. Our study offers further insights into the trade-offs between different RNA representations in practical applications and addresses a significant gap in evaluating deep learning models for RNA tasks.

==> sections/tmp.tex <==
\section{Introduction}
\label{sec:intro}


\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.72\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/teaser_a.pdf}
    \end{subfigure}
    \hspace{0.4cm}
    \begin{subfigure}[b]{0.1865\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/teaser_b.pdf}
    \end{subfigure}
    \vspace{-0.5em}
    \caption{\textbf{Overview of the study.} (a) Left panel: RNA sequences represented in 1D, 2D, and 3D structures, processed by Transformer, 2D GNN, and 3D GNN models. Analysis includes performance as measured by RMSE, robustness and generalization to sequencing noise, and performance under limited training data and partial labelings. (b) Right panel: Comparative performance of 1D, 2D, and 3D methods across experimental conditions. Histograms show RMSE performance, relative RMSE changes with increasing noise, and data requirements for optimal performance. Lower values indicate better performance in all metrics.}
    \vspace{-2em}
    \label{fig:teaser}
\end{figure}


% RNA is crucial; Developing methods to analyze RNA is important 
RNA plays a central role in the machinery of life, serving as a crucial intermediary between nucleotide and amino acid worlds~\citep{sahin2014mrna}. Beyond its messenger role, RNA is involved in diverse biological processes, including gene regulation, catalytic activity, and structural support within ribosomes~\citep{sharp2009centrality, strobel2016rna}. This versatility makes RNA a key target for fundamental biological research and therapeutic interventions. As our understanding of RNA complexity grows, so does the need for advanced computational tools for its analysis.

% Challenges of RNA analysis 
Modeling RNA is challenging due to its intricate secondary and tertiary structures, dynamic conformational changes, and interactions with cellular components~\citep{han2015advanced}. Furthermore, RNA analysis is hindered by the practical challenges of RNA data acquisition which include sequencing errors~\citep{ozsolak2011rna}, batch effects~\citep{tran2020benchmark}, incomplete sequencing~\citep{alfonzo2021call}, partial labeling~\citep{wayment2022deep}, and high costs of obtaining large labeled datasets~\citep{byron2016translating}. Moreover, RNA molecule can be represented in different ways: as a 1D nucleotide sequence, a 2D graph of base pairings, or a 3D atomic structure. Each representation highlights different aspects of RNA, presenting both opportunities and challenges for model design and selection (Fig.~\ref{fig:teaser}).

In this work, we systematically study the performance of various machine learning models for RNA property prediction, extending beyond traditional sequence-based approaches~\citep{he2021nucleic, soylu2023bert2ome, franke2022probabilistic} to include methods that process RNA with its 2D or 3D geometry. While 2D and 3D RNA representations offer potentially richer information, they also present unique challenges. In the absence of high-quality experimental data, accessing 2D or 3D RNA structures requires running prediction algorithms prone to noise and mistakes, especially in the presence of sequencing errors~\citep{schneider2023will, wang2023trrosettarna}. A few mutations in the nucleotide sequence owing to sequencing mistakes can hugely alter the 2D and 3D structure (Fig.~\ref{fig:rna_noise}), potentially undermining the benefit of using additional geometric context. Furthermore, real-world RNA datasets often suffer from partial labeling~\citep{wayment2022deep} and scarcity of training samples~\citep{wint2022kingdom}, which may affect geometry-aware methods differently than sequence-based approaches. These challenges raise a fundamental question: to what extent does explicit 2D and 3D geometry contribute to RNA property prediction, and under what circumstances might it offer advantages over geometry-free sequence models?

In this study, we seek to answer this question by making the following contributions: \textbf{(i)} we introduce a diverse collection of RNA datasets, including newly annotated 2D and 3D structures, covering a range of prediction tasks at both nucleotide and sequence levels across multiple species; \textbf{(ii)} we provide a unified testing environment to evaluate different types of machine learning models for RNA property prediction, including sequence models for 1D, graph neural networks for 2D, and equivariant geometric networks for 3D RNA representations; \textbf{(iii)} we conduct a comprehensive analysis of how different models perform under various conditions, such as limited data and labels, different types of sequencing errors, and out-of-distribution scenarios. We highlight the trade-offs and contexts in which each modeling approach is most effective, guiding researchers in selecting suitable models for specific RNA analysis challenges. 

Our study reveals several key insights: \textbf{(i)} 2D models generally outperform 1D models, with spectral GNNs reducing prediction error by about 12\%\ on average across all tasks, highlighting the importance of explicitly considering RNA structural information; \textbf{(ii)} 3D equivariant GNNs outperform 1D and some 2D methods in noise-free scenario but are sensitive to noise, exhibiting up to a 56\%\ decrease in prediction quality error under high sequencing error rates; \textbf{(iii)} geometry-free sequence models remain the most robust to sequencing noise, showing only a 14-27\%\ increase in prediction error compared to noise-free conditions, however they require around $2-5\times$ more training data to match the performance of geometry-aware models.








